A4 : Evading Learning-based Adblockers

Efforts by online ad publishers to circumvent traditional ad blockers towards regaining fiduciary benefits, have been demonstrably successful. As a result, there have recently emerged a set of adblockers that apply machine learning instead of manually curated rules and have been shown to be more robust in blocking ads on websites including social media sites such as Facebook. Among these, AdGraph is arguably the state-of-the-art learning-based adblocker. In this paper, we develop A4, a tool that intelligently crafts adversarial samples of ads to evade AdGraph. Unlike the popular research on adversarial samples against images or videos that are considered less- to un-restricted, the samples that A4 generates preserve application semantics of the web page, or are actionable. Through several experiments we show that A4 can bypass AdGraph about 60% of the time, which surpasses the state-of-the-art attack by a significant margin of 84.3%; in addition, changes to the visual layout of the web page due to these perturbations are imperceptible. We envision the algorithmic framework proposed in A4 is also promising in improving adversarial attacks against other learning-based web applications with similar requirements.

==> docs/abs.tex <==

Efforts by ad publishers to circumvent 
traditional ad blockers towards regaining fiduciary benefits, 
have been demonstrably successful. Because of this,
there have recently emerged a set of ad blockers that apply machine
learning instead of manually curated rules and these have been shown
to be more robust in blocking ads. Among these, AdGraph which uses rich
contextual information to perform classifications,  is 
the state of the art ad blocker. In this paper, we develop a novel
tool called \tool, which 
intelligently crafts adversarial samples of ads that evade
AdGraph. Unlike the popular research on adversarial samples against images
or videos, the samples that \tool generates preserve constraints that
accompany the domain of application i.e., it preserves application semantics of
the web page. Via several experiments we show that ads that are manipulated
with \tool can bypass AdGraph more than {\color{black} 60 \%} of the time; in
addition, changes to the visual layout of the webpage due to these perturbations
are imperceptible.

